Dynamic Approximate All-Pairs Shortest Paths: Breaking the O(mn) Barrier and Derandomization

We study dynamic $(1+\epsilon)$-approximation algorithms for the all-pairs shortest paths problem in unweighted undirected $n$-node $m$-edge graphs under edge deletions. The fastest algorithm for this problem is a randomized algorithm with a total update time of $\tilde O(mn/\epsilon)$ and constant query time by Roditty and Zwick [FOCS 2004]. The fastest deterministic algorithm is from a 1981 paper by Even and Shiloach [JACM 1981]; it has a total update time of $O(mn^2)$ and constant query time. We improve these results as follows: (1) We present an algorithm with a total update time of $\tilde O(n^{5/2}/\epsilon)$ and constant query time that has an additive error of $2$ in addition to the $1+\epsilon$ multiplicative error. This beats the previous $\tilde O(mn/\epsilon)$ time when $m=\Omega(n^{3/2})$. Note that the additive error is unavoidable since, even in the static case, an $O(n^{3-\delta})$-time (a so-called truly subcubic) combinatorial algorithm with $1+\epsilon$ multiplicative error cannot have an additive error less than $2-\epsilon$, unless we make a major breakthrough for Boolean matrix multiplication [Dor et al. FOCS 1996] and many other long-standing problems [Vassilevska Williams and Williams FOCS 2010]. The algorithm can also be turned into a $(2+\epsilon)$-approximation algorithm (without an additive error) with the same time guarantees, improving the recent $(3+\epsilon)$-approximation algorithm with $\tilde O(n^{5/2+O(\sqrt{\log{(1/\epsilon)}/\log n})})$ running time of Bernstein and Roditty [SODA 2011] in terms of both approximation and time guarantees. (2) We present a deterministic algorithm with a total update time of $\tilde O(mn/\epsilon)$ and a query time of $O(\log\log n)$. The algorithm has a multiplicative error of $1+\epsilon$ and gives the first improved deterministic algorithm since 1981. It also answers an open question raised by Bernstein [STOC 2013].

==> putting_together.tex <==
\subsection{Putting Everything Together: $ \tilde O(n^{5/2})$-total-time Algorithm for $({1+\epsilon}, 2)$- and $(2+\epsilon, 0)$-approximate APSP}\label{sec:putting together for faster algorithms}

In the following we show how the monotone ES-tree of \Cref{thm:monotone ES tree} together with the locally persevering emulator of \Cref{thm:emulator} can be used to obtain $ (1+\epsilon, 2) $- and $ (2+\epsilon, 0) $-approximate decremental APSP algorithms with $ \tilde O (n^{5/2} / \epsilon^2) $ total update time.

We will proceed as follows: we first show, as a simple consequence of the previous two parts of this sections, how to maintain a $ (1+\epsilon, 2) $-approximate monotone ES-tree (\Cref{cor:concrete_monotone_ES_tree}).
This monotone ES-tree provides us with $ (1 + \epsilon, 2) $-approximate \emph{single-source} shortest paths.
The main work now is to extend this to an algorithm for $ (1 + \epsilon, 2) $-approximate \emph{all-pairs} shortest paths.
We define an {\em approximate} version of the center cover data structure (\Cref{def:approximate_center_cover}) and show how such a data structure can be turned into an approximate decremental APSP algorithm (\Cref{lem:approximate_centers_data_structure_to_APSP}).
Afterwards we show that a $ (1+\epsilon, 2) $-approximate center cover data structures exists (\Cref{lem:center_cover_for_additive_two}) by using \Cref{cor:concrete_monotone_ES_tree}.
We can use this data structure to obtain a $ (1+\epsilon, 2) $-approximate APSP algorithm (due to \Cref{lem:approximate_centers_data_structure_to_APSP}).
The $ (2+\epsilon, 0) $-approximate algorithm then follows as a corollary from the $ (1+\epsilon, 2) $-approximate algorithm.
Our arguments mainly follow Roditty and Zwick~\cite{RodittyZ12} with necessary adaptions for \emph{approximate} instead of exact center cover data structures.
The most interesting technical details are the following:
\begin{itemize}
\item In their algorithm, Roditty and Zwick keep a set of nodes $ U $ (which we call centers) such that every node (that is in a sufficiently large connected component) is ``close'' to some node in $ U $.
To be able to efficiently find a close center for every node, they maintain, for every node, the nearest node in the set of centers.
However, it is sufficient to return \emph{any} center that is close.
\item The $ (1+\epsilon, 2) $-approximate center cover data structure does \emph{not} directly imply a $ (1+\epsilon, 2) $-approximate decremental APSP algorithm, but gives a slightly worse approximation.
This only causes a problem for relatively small distances.
Therefore we can resolve this issue by maintaining a monotone ES-tree of small depth for every node.
\item The $ (2+\epsilon, 0) $-approximation follows from the $ (1 + \epsilon, 2) $-approximation by the following simple observation: we can easily find out whether the distance of two nodes is $ 1 $ by checking whether there is an edge between the two nodes in the current graph.
\end{itemize}


First, we show a simple consequence of the main results of the previous two parts in this section (\Cref{thm:emulator} and \Cref{thm:monotone ES tree}).
The monotone ES-tree gives a $ (1 + \epsilon, 2) $-approximation of the true distance if we run it on the emulator we described in \Cref{sec:emulator}.
This is a key tool for the following results.

\begin{corollary}[$ (1 + \epsilon, 2) $-approximate monotone ES-tree]\label{cor:concrete_monotone_ES_tree}
Given a dynamic graph $ \cG = (G_i)_{0 \leq i \leq k} $, an integer $ \Q $, and a distinguished node $ \treeroot $, we can maintain a $ (1 + \epsilon, 2) $-approximate monotone ES-tree rooted at $ \treeroot $ up to depth $ \Q $ under $ k $ edge deletions.
After each deletion $ i $, the data structure can provide an estimate $ \delta (x, \treeroot) $ of the distance $ \dist_{G_i} (x, \treeroot) $ in constant time such that $ \dist_{G_i} (x, \treeroot) \leq \delta (x, \treeroot) $.
Furthermore, if $ \dist_{G_i} (x, \treeroot) \leq \Q $, then $ \delta (x, \treeroot) \leq (1 + \epsilon) \dist_{G_i} (x, \treeroot) + 2 $  with high probability.
The total update time of this data structure is $ O ( n^{3/2} \log{n} / \epsilon + n^{3/2} \Q \log^2{n} + m n^{1/2} \log{n} / \epsilon) $.
\end{corollary}

The term $ m n^{1/2} \log{n} / \epsilon $ in the running time stated above comes from the time needed for maintaining an emulator.
If we want to maintain several $ (1 + \epsilon, 2) $-approximate monotone ES-trees with different root nodes, then the total update time for maintaining this emulator only has to be counted once.
We will consider this fact when we apply this result later on.

\begin{proof}[Proof of \Cref{cor:concrete_monotone_ES_tree}]
Let $ \cH $ denote the $ (1, 2, 2/\epsilon) $-locally persevering emulator of \Cref{thm:emulator}.
The total update time for maintaining $ \cH $ is $ O (m n^{1/2} \log{n} / \epsilon) $.
We maintain a monotone ES-tree rooted at $ \treeroot $ with distance range parameter $ \Q $ on $ \cH $, as given by \Cref{thm:monotone ES tree}.
Let $ \delta (x, \treeroot) $ denote the level of the node $ x $ in the monotone ES-tree of $ \treeroot $ after deletion $ i $.
By \Cref{thm:monotone ES tree} we have $ \dist_{G_i} (x, c) \leq \delta (x, c) $, and furthermore, if $ \dist_{G_i} (x, c) \leq \Q $, then
\begin{equation*}
\delta_{G_i} (x, c) \leq (1 + 2 / (2 / \epsilon)) \dist_{G_i} (x, c) + 2 = (1 + \epsilon) \dist_{G_i} (x, c) + 2 \, .
\end{equation*}
By \Cref{thm:emulator}, the number of edges ever contained in the emulator is $ | E_k (\cH) | = O (n^{3/2} \log{n}) $ and the total number of updates in $ \cH $ is $ \phi_k (\cH) = O (n^{3/2} \log{n} / \epsilon) $.
Therefore, by \Cref{thm:monotone ES tree}, the total update time of the monotone ES-tree (without the time for maintaining the emulator $ \cH $) is
\begin{equation*}
O \left( \phi_k(\cH) + \sum_{x \in V} \deg_{\cH} (x) \Q \log{n} \right) = O ( n^{3/2} \log{n} / \epsilon + n^{3/2} \Q \log^2{n} ) \, .
\end{equation*}
Together with the time needed for maintaining $ \cH $, this gives a total update time of
\begin{equation*}
O ( n^{3/2} \log{n} / \epsilon + n^{3/2} \Q \log^2{n} + m n^{1/2} \log{n} / \epsilon) \, .
\end{equation*}
\end{proof}

We now define an approximate version of the center cover data structure and show how such a data structure can be turned into an approximate decremental APSP algorithm.
We modify the notions of a center cover and a center cover data structure we gave in \Cref{sec:Roditty_Zwick_framework}, where we reviewed the algorithmic framework of Roditty and Zwick.

\begin{definition}[Approximate center cover]
Let $ U $ be a set of nodes of a graph $ G $, let $ \q $ be a positive integer, the \emph{cover range}, and let $ \alpha \geq 1 $ and $ \beta \geq 0 $.
We say that a node $ x $ is \emph{$ (\alpha, \beta) $-covered} by a node $ \cen \in U $ if $ \dist_G (x, \cen) \leq \alpha \q + \beta $.
We say that $ U $ is an \emph{$ (\alpha, \beta) $-approximate center cover of $ G $ with parameter $ \q $} if every node $ x $ that is in a connected component of size at least $ \q $ is $ (\alpha, \beta) $-covered by some node $ \cen \in U $.
\end{definition}

\begin{definition}\label{def:approximate_center_cover}
An \emph{$ (\alpha, \beta) $-approximate center cover data structure}  with \emph{cover range parameter $ \q $} and \emph{distance range parameter $ \Q $} for a decremental graph $ \cG = (G_i)_{0 \leq i \leq k} $ maintains a set of \emph{centers} $ \C = \{ 1, 2, \ldots, l \} $ and a set of nodes $ U = \{ \cen^1, \cen^2, \ldots, \cen^l \} $ such that, for every $ 0 \leq i \leq k $, $ U $ is an $ (\alpha, \beta) $-approximate center cover of $ G_i $ with parameter $ \q $.
For every center $ j \in \C $ we call $ \cen^j $ the \emph{location} of center $ j $ and for every node $ x $ we say that $ x $ is $ (\alpha, \beta) $-covered by $ j $ if $ x $ is $ (\alpha, \beta) $-covered by $ \cen^j $.
The data structure provides the following update operations:
\begin{itemize}
\item $ \Call{Initialize}{G_0, \q, \Q} $: Initialize the data structure
\item $ \Call{Delete}{u, v} $: Delete the edge $ (u, v) $ from the current graph
\end{itemize}
The data structure provides the following query operations, applied on the current graph $ G_i $ after the $i$-th edge deletion:
\begin{itemize}
\item $ \Call{Distance}{j, x} $: Return an estimate $ \delta (\cen^j, x) $ of the distance between the current location $ \cen^j $ of center $ j $ and the node $ x $ such that $ \delta (\cen^j, x) \leq \alpha \dist_{G_i} (\cen^j, x) + \beta $, provided that $ \dist_{G_i} (\cen^j, x) \leq \Q $.
If $ \dist_{G_i} (\cen^j, x) > \Q $, then either return $ \delta (\cen^j, x) = \infty $ or return $ \delta (\cen^j, x) \leq \alpha \dist_{G_i} (\cen^j, x) + \beta $.
\item $ \Call{FindCenter}{x} $ If $ x $ is in a connected component of size at least $ \q $, then return a center $ j $ (with current location $ \cen^j $) such that $ \dist_{G_i} (x, \cen^j) \leq \alpha \q + \beta $.
If $ x $ is in a connected component of size less than $ \q $, then either return $ \bot $ or return a center $ j $ such that $ \dist_{G_i} (x, \cen^j) \leq \alpha \q + \beta $.
\end{itemize}
\end{definition}

We now show why the approximate center cover data structure is useful.
If one can obtain an approximate center cover data structure, then one also obtains an approximate decremental APSP algorithm with slightly worse approximation guarantee.
The proof of this observation follows~\cite{RodittyZ12}.

\begin{lemma}[Approximate center cover implies approximate APSP]\label{lem:approximate_centers_data_structure_to_APSP}
Assume that for all parameters $ \q $ and $ \Q $ such that $ \q \leq \Q $ there is an $ (\alpha, \beta) $-approximate center cover data structure that has constant query time and a total update time of $ T(n, m, \q, \Q) $.
Then, for every $ \epsilon \leq 1 $, there is an $ (\alpha + 2 \alpha^2 \epsilon, 2 \beta + 2 \alpha \beta) $-approximate decremental APSP algorithm with $ O(\log{\log n}) $ query time and a total update time of $ \sum_p T(n, m, \qp, \Qp) $ where $ \qp = \epsilon 2^p $ and $ \Qp = \alpha \epsilon 2^p + \beta + 2^{p+1} $ (for $ 0 \leq p \leq \lfloor \log{n} \rfloor $).

The query time can be reduced to $ O (1) $ if there is an $ (\alpha', \beta') $-approximate decremental APSP algorithm for some constants $ \alpha' $ and $ \beta' $ with constant query time (at the cost of additional update time for this algorithm).
\end{lemma}

\begin{proof}
The algorithm uses $ \lceil \log n \rceil $ many layers where the $ p $-th layer is responsible for the distance range from $ 2^p $ to $ 2^{p+1} $. 
For each layer the algorithm maintains a center cover data structure using the parameters $ \qp = \epsilon 2^p $ and $ \Qp = 2^{p+1} + \alpha \epsilon 2^p + \beta $.
For all nodes $ x $ and $ y $, let $ \delta (x, y) $ denote the estimate of the distance between $ x $ and $ y $ provided by the center cover data structure.
Let $ i $ be the index of the last deletion.

For every layer $ p $, we can compute a distance estimate $ \delta_p' (x, y) $ for two nodes $ x $ and $ y $ as follows.
Using the center cover data structure, we first check whether there is some center $ j $ with location $ \cen^j $ that $ (\alpha, \beta) $-covers $ x $, i.e., $ \dist_{G_i} (x, \cen^j) \leq \alpha \qp + \beta $.
If $ x $ is not $ (\alpha, \beta) $-covered by any center we set $ \delta_p' (x, y) = \infty $.
Otherwise we query the center cover data structure to get estimates $ \delta_p (\cen^j, x) $ and $ \delta_p (\cen^j, y) $ of the distances from $ \cen^j $ to $ x $ and $ y $, respectively.
(Remember that these distance estimates might be $ \infty $.)
We now set $ \delta_p' (x, y) = \delta_p (\cen^j, x) + \delta_p (\cen^j, y) $.
Note that, given $ p $, we can compute $ \delta_p' (x, y) $ in constant time.
The query procedure will rely on three properties of the distance estimate $ \delta_p' (x, y) $.
\begin{enumerate}
\item The distance estimate never under-estimates the true distance, i.e., $ \delta_p' (x, y) \geq \dist_{G_i} (x, y) $.
\item If $ \dist_{G_i} (x, y) \geq 2^p $ and $ \delta_p' (x, y) \neq \infty $, then $\delta_p' (x, y) \leq (\alpha + 2 \alpha^2) \dist_{G_i} (x, y) + 2 \beta + 2 \alpha \beta $.
\item If $ x $ is in a connected component of size at least $ \qp $ and $ \dist_{G_i} (x, y) \leq 2^{p+1} $, then $ \delta_p' (x, y) \neq \infty $.
\end{enumerate}

The first property is clearly true if $ \delta_p' (x, y) = \infty $ and otherwise follows by applying the triangle inequality (note that $ \dist_{G_i} (\cen^j, y) \leq \delta_p (\cen^j, y) $ in any case):
\begin{equation*}
\dist_{G_i} (x, y) \leq \dist_{G_i} (\cen^j, x) + \dist_{G_i} (\cen^j, y) \leq \delta_p (\cen^j, x) + \delta_p (\cen^j, y) = \delta_p' (x, y) \, .
\end{equation*}
Thus, $ \delta_p' (x, y) $ never under-estimates the true distance.
For the second property we remark that if $ \delta_p' (x, y) \neq \infty $, it must be the case that we have found a center $ j $ with location $ \cen^j $ that $ (\alpha, \beta) $-covers $ x $.
Therefore $ \dist_{G_i} (x, \cen^j) \leq \alpha \qp + \beta $.
Furthermore it must be the case that $ \delta_p (x, \cen^j) \neq \infty $ and $ \delta_p (\cen^j, y) \neq \infty $ and therefore $ \delta_p (x, \cen^j) \leq \alpha \dist_{G_i} (x, \cen^j) + \beta $ and $ \delta_p (\cen^j, y) \leq \alpha \dist_{G_i} (\cen^j, y) + \beta $.
Now simply consider the following chain of inequalities:
\begin{align*}
\delta_p' (x, y) = \delta_p (x, \cen^j) + \delta_p (\cen^j, y) &\leq \alpha (\dist_{G_i} (\cen^j, x) + \dist_{G_i} (\cen^j, y)) + 2 \beta \\
 &\leq \alpha (\dist_{G_i} (\cen^j, x) + \dist_{G_i} (\cen^j, x) + \dist_{G_i} (x, y)) + 2 \beta \\
 &= \alpha (2 \dist_{G_i} (\cen^j, x) + \dist_{G_i} (x, y)) + 2 \beta \\
 &\leq \alpha (2 \alpha \qp + 2\beta + \dist_{G_i} (x, y)) + 2 \beta \\
 &= \alpha (2 \alpha \epsilon 2^p + 2\beta + \dist_{G_i} (x, y)) + 2 \beta \\
 &\leq \alpha (2 \alpha \epsilon \dist_{G_i} (x, y) + 2\beta + \dist_{G_i} (x, y)) + 2 \beta \\
 &= (\alpha + 2 \alpha^2 \epsilon) \dist_{G_i} (x, y) + 2 \beta + 2 \alpha \beta
\end{align*}
We now prove the third property.
If $ x $ is in a component of size at least $ \qp $, then it is covered by some center with location $ \cen^j $ and we have 
\begin{equation*}
\dist_{G_i} (\cen^j, x) \leq \alpha \qp + \beta = \alpha \epsilon 2^p + \beta \leq \Qp
\end{equation*}
as well as
\begin{equation*}
\dist_{G_i} (\cen^j, y) \leq \dist_{G_i} (\cen^j, x) + \dist_{G_i} (x, y) \leq \alpha \epsilon 2^p + \beta + 2^{p+1} = \Qp \, .
\end{equation*}
Therefore we get $ \delta_p (\cen^j, x) \leq \alpha \dist_{G_i} (\cen^j, x) + \beta < \infty $ as well as $ \delta_p (\cen^j, y) < \infty $ which implies $ \delta_p' (x, y) \neq \infty $ as desired.

A query time of $ O (\log{n}) $ is immediate as we can simply return the minimum of all distance estimates $ \delta_p' (x, y) $.
A query time of $ O (\log {\log{n}}) $ is possible because of the following idea:
If $ \dist_{G_i} (x, y) \neq \infty $, it is sufficient to find the minimum index $ p $ such that $ \delta_p' (x, y) \neq \infty $.
This minimum index can be found by performing binary search over all $ \log{n} $ possible indices.
Furthermore, the query time can be reduced to $ O(1) $ if there is a second $ (\alpha', \beta') $-approximate decremental APSP algorithm with query time $ O(1) $ for some constants $ \alpha' $ and $ \beta' $, 
We first compute the distance estimate $ \delta'' (x, y) $ of the second algorithm for which we know that $ \dist_{G_i} (x, y) \in [ \delta'' (x, y) / \alpha' - \beta', \delta'' (x, y) ] $.
Now there is only a constant number of indices $ p $ such that $ \{ 2^p, \ldots, 2^{p+1} \} \cap [ \delta'' (x, y) / \alpha' - \beta', \delta'' (x, y) ] \neq \emptyset $.
For every such index we compute $ \delta_p' (x, y) $ and return the minimum distance estimate obtained by this process.
\end{proof}

Our next goal is to obtain a useful approximate center cover data structure.
We show the existence of $ (1 + \epsilon, 2) $-approximate center cover data structures with favorable running time.
Here we use the $ (1 + \epsilon, 2) $-approximate monotone ES-tree of \Cref{cor:concrete_monotone_ES_tree} together with a well-known idea of finding a center cover by random sampling of nodes.
Again, the proof is rather straightforward.

\begin{lemma}[Existence of $ (1 + \epsilon, 2) $-approximate center cover data structure]\label{lem:center_cover_for_additive_two}
For all parameters $ \q $ and $ \Q $ such that $ \q \leq \Q $, there is a $ (1 + \epsilon, 2) $-approximate center cover data structure that maintains a $ (1 + \epsilon, 2) $-approximate center cover with high probability.
It has constant query time and a total update time of
\begin{equation*}
O(n^{5/2} \log^2{n} / (\epsilon \q) +  n^{5/2} \log^3{n} \Q / \q + m n^{1/2} \log{n} / \epsilon) \, .
\end{equation*}
\end{lemma}

The term $ m n^{1/2} \log{n} / \epsilon $ in the running time stated above comes from the time needed for maintaining an emulator.
If we want to maintain more than one $ (1 + \epsilon, 2) $-approximate center cover data structure, then the total update time for maintaining the emulator only has to be counted once. We will consider this fact when we apply this result later on.

\begin{proof}[Proof of \Cref{lem:center_cover_for_additive_two}]
It is well-known (see for example~\cite{UllmanY91} and~\cite{RodittyZ12}) that, by random sampling, we can obtain a set $ U = \{ \cen^1, \cen^2, \ldots, \cen^l \} $ of size $ O (n \log{n} / \q) $ that is a center cover of $ G_i $ for every $ i \leq k $.
Clearly, every center cover is also an $ (\alpha, \beta) $-approximate center cover.
Thus, $ U $ is an $ (\alpha, \beta) $-approximate center cover of $ G_i $ for every  $ i \leq k $.
Throughout all deletions, the set $ \C = \{ 1, 2, \ldots, l \} $ will serve as the set of centers and each center $ j $ will always be located at the same node $ \cen^j $.

For every center $ j $, we maintain the $ (1 + \epsilon, 2) $-approximate monotone ES-tree of \Cref{cor:concrete_monotone_ES_tree} rooted at $ \cen^j $ up to depth $ \Q $.
As there are $ O (n \log{n} / \q) $ centers, the total update time for maintaining all the monotone ES-trees is
\begin{equation*}
O ((n^{3/2} \log{n} / \epsilon + n^{3/2} \log^2{n} \Q) n \log{n} / \q + m n^{1/2} \log{n} / \epsilon)
\end{equation*}
which is equal to
\begin{equation*}
O(n^{5/2} \log^2{n} / (\epsilon \q) +  n^{5/2} \log^3{n} \Q / \q + m n^{1/2} \log{n} / \epsilon) \, .
\end{equation*}
Note that the second term in the running time of \Cref{cor:concrete_monotone_ES_tree} does \emph{not} have to be multiplied by the number of centers because it comes from maintaining an emulator that all monotone ES-trees can share.
Furthermore, for every node $ x $ we maintain a list of centers that cover $ x $, i.e., a list containing every $ j \in \C $ such that the level of $ x $ in the monotone ES-tree of $ \cen^j $ is at most $ (1 + \epsilon) \q + 2 $.
To maintain this list we just have to observe the level increases in each monotone ES-tree.
If for some center $ j $ and some node $ x $ the level of $ x $ in the monotone ES-tree rooted at $ \cen^j $ exceeds the threshold $  (1 + \epsilon) \q + 2 $ we remove $ j $ from the list of $ x $.
Therefore we can charge the running time for maintaining this list to the level-increases in the monotone ES-tree, which means that the running time for maintaining the list is already included in the total update time stated above.

We now show how to answer queries of a center cover data structure, as specified in \Cref{def:approximate_center_cover}, in constant time.
Let $ i $ be the index of the last deletion.
For every node $ x $ and every center $ j $, let $ \delta (x, \cen^j) $ denote the estimate of the distance of $ x $ to the location of center $ j $ as returned by the monotone ES-tree rooted at $ \cen^j $.
Given a center $ j $ and a node $ x $ we answer a query for the distance of $ x $ to $ \cen^j $ by returning $ \delta (\cen^j, y) $ which gives a $ (1+\epsilon, 2) $-approximation of the true distance by \Cref{cor:concrete_monotone_ES_tree}.
Given a node $ x $, we answer a query for finding a nearby center by returning any center $ j $ in the list of centers of $ x $.
If this list is empty we return $ \bot $.
Note that for every center $ j $ in the list we know that $ \dist_{G_i} (x, \cen^j) \leq (1 + \epsilon) \q + 2 $ as required because $ \dist_{G_i} (x, \cen^j) \leq \delta (x, \cen^j) $ by \Cref{cor:concrete_monotone_ES_tree}.
If $ x $ is in a connected component of size at most $ \q $ we can ensure that we really find a center $ j $ in that list because, by our random choice of centers, we have $ \dist_{G_i} (x, \cen^j) \leq \q $ for some center $ j $ with high probability in that case.
If $ \dist_{G_i} (x, \cen^j) \leq \q $, then also $ \dist_{G_i} (x, \cen^j) \leq \Q $ and by \Cref{cor:concrete_monotone_ES_tree} we get $ \delta (x, \cen^j) \leq (1 + \epsilon) \dist_{G_i} (x, \cen^j) + 2 \leq (1 + \epsilon) \q + 2 $.
Therefore the list of centers of $ x $ contains $ j $.
\end{proof}

Finally we show how to obtain the $ (1 + \epsilon, 2) $-approximate decremental APSP algorithm.
We combine the $ (1 + \epsilon, 2) $-approximate center cover data structure of \Cref{lem:center_cover_for_additive_two} with the approximate APSP algorithm of \Cref{lem:approximate_centers_data_structure_to_APSP} that uses this data structure.
However, the approximation guarantee we get from this algorithm is not as good as desired because the additive errors accumulate.
Therefore we need a special treatment of relatively short distances.
It is a standard technique to maintain small-depth shortest paths trees to handle these cases.
We can use our monotone ES-tree for this purpose.

\begin{theorem}[Main result of \Cref{sec:faster}: Randomized $(1+\epsilon, 2)$-approximation with truly-subcubic total update time]\label{thm:main_APSP_approximation}
Given a decremental graph $ \cG = (G_i)_{0 \leq i \leq k} $ and  $ 0< \epsilon \leq 1 $, there is a $ (1 + \epsilon, 2) $-approximate decremental APSP algorithm with constant query time and a total update time of $ O ( n^{5/2} (\log^2{n}) / \epsilon^2 + n^{5/2} (\log^4{n}) / \epsilon ) $.
The approximation guarantee holds with high probability.
\end{theorem}

\begin{proof}
By \Cref{lem:center_cover_for_additive_two} there is a $ (1 + \epsilon, 2) $-approximate center cover data structure that has constant query time and a total update time of
\begin{equation*}
O(n^{5/2} \log^2{n} / (\epsilon \q) +  n^{5/2} \log^3{n} \Q / \q + m n^{1/2} \log{n} / \epsilon) \, .
\end{equation*}
By applying \Cref{lem:approximate_centers_data_structure_to_APSP}, this data structure gives us an an approximate decremental APSP algorithm.
The parameters used by the algorithm are $ \qp = \epsilon 2^p $ and $ \Qp = (1 + \epsilon) \epsilon 2^p + 2 + 2^{p+1} \leq 2^{p+3} $ (for $ 0 \leq p \leq \log{n} $) and therefore its total running time is\footnote{The term $ m n^{1/2} \log{n} $ shows up in the running time only once because it is the time for maintaining an emulator that can be shared by all $ \log{n} $ layers.}
\begin{equation*}
O \left( \sum_{p=0}^{\log{n}} \left( n^{5/2} \log^2{n} / (\epsilon \qp) +  n^{5/2} \log^3{n} \Qp / \qp \right) + m n^{1/2} \log{n} / \epsilon \right) \, .
\end{equation*}
Now consider the following arithmetic simplifications:
\begin{align*}
O \left( \sum_{p=0}^{\log{n}} n^{5/2} \log^2{n} / (\epsilon \qp) \right) &= O \left( \sum_{p=0}^{\log{n}} n^{5/2} \log^2{n} / (\epsilon^2 2^p) \right) \\
 &= O \left( \frac{n^{5/2} \log^2{n}}{\epsilon^2} \sum_{p=0}^{\log{n}} \frac{1}{2^p} \right) = O \left( n^{5/2} \log^2{n} / \epsilon^2 \right) \\
O \left( \sum_{p=0}^{\log{n}} n^{5/2} \log^3{n} \Qp/ \qp \right) &= O \left( \sum_{p=0}^{\log{n}} n^{5/2} \log^3{n} 2^{p+3} / (\epsilon 2^p) \right) \\
 &= O \left( \sum_{p=0}^{\log{n}} 8 n^{5/2} \log^3{n} / \epsilon \right) = O \left( n^{5/2} \log^4{n} / \epsilon \right)
\end{align*}
Therefore the total update time of the algorithm provided by \Cref{lem:approximate_centers_data_structure_to_APSP} can also be expressed as
\begin{equation}
O \left( n^{5/2} \log^2{n} / \epsilon^2 + n^{5/2} \log^4{n} / \epsilon + m n^{1/2} \log{n} / \epsilon \right) \, . \label{eq:running_time_APSP}
\end{equation}

The query time of the algorithm provided by \Cref{lem:approximate_centers_data_structure_to_APSP} can be reduced to $ O (1) $.
The reason is that Bernstein and Roditty~\cite{BernsteinR11} provide, for example, a decremental $ (5 + \epsilon', 0) $-approximate APSP algorithm for some constant $ \epsilon' $.
The total update time of the Bernstein-Roditty algorithm is
\begin{equation}
\tilde O \left( n^{2 + 1/3 + O (1/\sqrt{\log{n}})} \right) \label{eq:running_time_constant_approximation}
\end{equation}
which is well within $ O (n^{5/2}) $.

Let $ i $ be the index of the last edge deletion.
The approximation guarantee of the algorithm provided by \Cref{lem:approximate_centers_data_structure_to_APSP} with $ \alpha = 1 + \epsilon $ and $ \beta = 2 $ is
\begin{equation*}
\dist_{G_i} (x, y) \leq \delta (x, y) \leq (1 + \epsilon + 2 (1 + \epsilon)^2 \epsilon) \cdot \dist_{G_i} (x, y) + 4 + 4 (1 + \epsilon) \, .
\end{equation*}
Using $ \epsilon \leq 1 $ we get
\begin{equation*}
\delta (x, y) \leq (1 + 9 \epsilon ) \dist_{G_i} (x, y) + 12 \, .
\end{equation*}
By running the algorithm with $ \epsilon' = \epsilon / 18 $ we get
\begin{equation*}
\delta (x, y) \leq (1 + \epsilon/2 ) \dist_{G_i} (x, y) + 12 \, .
\end{equation*}
It is left to show how to get the approximation down to $ (1 + \epsilon, 2) $.
Here we need a special treatment of relatively small distances.

Note that if $ \dist_{G_i} (x, y) \geq 24 / \epsilon $ we get
\begin{equation*}
\delta (x, y) \leq (1 + \epsilon/2 ) \dist_{G_i} (x, y) + 12 \leq (1 + \epsilon/2 ) \dist_{G_i} (x, y) + \epsilon \dist_{G_i} (x, y) / 2 = (1 + \epsilon ) \dist_{G_i} (x, y) \, .
\end{equation*}
We now show how to deal with pairs of nodes whose distance is relatively small.
In addition to the algorithm above, we maintain the $ (1 + \epsilon, 2) $-approximate monotone ES-tree of \Cref{cor:concrete_monotone_ES_tree} with parameter $ \Q = 24 / \epsilon $ rooted at every node.
The total update time for these additional monotone ES-trees is\footnote{The term $ m n^{1/2} \log{n} $ shows up in the running time only once because it is the time for maintaining an emulator that can be shared by all monotone ES-trees.}
\begin{equation*}
O ( (n^{3/2} \log{n} / \epsilon + n^{3/2} \Q \log^2{n}) n + m n^{1/2} \log{n} / \epsilon)
\end{equation*}
which is equal to
\begin{equation}
O ( n^{5/2} \log{n} / \epsilon + n^{5/2} \log^2{n} / \epsilon + m n^{1/2} \log{n} / \epsilon) \, . \label{eq:running_time_small_depth_trees}
\end{equation}
For every pair of nodes $ x $ and $ y $, let $ \delta' (x, y) $ denote the distance estimate obtained by querying the distance to $ y $ in the monotone ES-tree rooted at $ x $ of depth $ \Q = 24 / \epsilon $ (this query takes constant time).
If $ \dist_{G_i} (x, y) \leq 24 / \epsilon $, then by \Cref{thm:monotone ES tree} we can be sure that $ y $ is contained in the monotone ES-tree root at $ x $ and we get
\begin{equation*}
\dist_{G_i} (x, y) \leq \delta' (x, y) \leq (1 + \epsilon) \dist_{G_i} (x, y) + 2 \, .
\end{equation*}
Thus, the minimum between $ \delta (x, y) $ and $ \delta' (x, y) $, the distance estimates of the APSP algorithm of \Cref{lem:approximate_centers_data_structure_to_APSP} and the additional ES-trees, respectively, provides a $ (1+\epsilon, 2) $-approximation of the distance $ \dist_{G_i} (x, y) $.

The query time of the overall algorithm is obviously constant because we just have to return the minimum of two data structures with constant query time.
Now for calculating the overall running time, observe that $ m \leq n^2 $ and thus $ O (m n^{1/2} \log{n} / \epsilon) = O (n^{5/2} \log{n} / \epsilon) $.
The dominating terms of \eqref{eq:running_time_APSP}, \eqref{eq:running_time_constant_approximation}, and \eqref{eq:running_time_small_depth_trees} are $ n^{5/2} \log^2{n} / \epsilon^2 $ and $  n^{5/2} \log^4{n} / \epsilon $ and therefore the total update time is
\begin{equation*}
O \left( n^{5/2} \log^2{n} / \epsilon^2 + n^{5/2} \log^4{n} / \epsilon \right) \, .
\end{equation*}
\end{proof}

The $ (2 + \epsilon, 0) $-approximate decremental APSP algorithm now follows as a corollary.
We simply need the following observation:
if the distance between two nodes is $ 1 $, then we can answer queries for their distance exactly by checking whether they are connected by an edge.

\begin{corollary}[Randomized $(2+\epsilon, 0)$-approximation with truly-subcubic total update time]\label{thm:2-approx}
Given a decremental graph $ \cG = (G_i)_{0 \leq i \leq k} $ and  $ 0< \epsilon \leq 1 $, there is a $ (2 + \epsilon, 0) $-approximate decremental APSP algorithm with constant query time and a total update time of $ O ( n^{5/2} (\log^2{n}) / \epsilon^2 + n^{5/2} (\log^4{n}) / \epsilon ) $.
The approximation guarantee holds with high probability.
\end{corollary}

\begin{proof}
By running the algorithm of \Cref{thm:main_APSP_approximation} we can, after each edge deletion $ i $, for all nodes $ x $ and $ y $, query for a distance estimate $ \delta (x, y) $ in constant time that satisfies:
\begin{equation*}
\dist_{G_i} (x, y) \leq \delta (x, y) \leq (1 + \epsilon) \dist_{G_i} (x, y) + 2
\end{equation*}
Note that if $ \dist_{G_i} (x, y) \geq 2 $, then
\begin{equation*}
\dist_{G_i} (x, y) \leq (1 + \epsilon) \dist_{G_i} (x, y) + 2 \leq (1 + \epsilon) \dist_{G_i} (x, y) + \dist_{G_i} (x, y) = (2 + \epsilon) \dist_{G_i} (x, y) \, .
\end{equation*}
If $ \dist_{G_i} (x, y) < 2 $, then we actually have $ \dist_{G_i} (x, y) \leq 1 $ because $ G_i $ is an unweighted graph.
A distance of $ 1 $ simply means that there is an edge connecting $ x $ and $ y $ in $ G_i $.
Since the adjacency matrix of $ \cG $ is maintained anyway, we can find out in constant time whether $ \dist_{G_i}(x, y) = 1 $.
By setting, for all nodes $ x $ and $ y $,
\begin{equation*}
\delta' (x, y) = \begin{cases}
0 & \text{if $ x = y $} \\
1 & \text{if $ (x, y) \in E (G_i) $} \\
\delta (x, y) & \text{otherwise}
\end{cases}
\end{equation*}
we get $ \dist_{G_i} (x, y) \leq \delta' (x, y) \leq (2 + \epsilon) \dist_{G_i} (x, y) $.
Clearly, this algorithm can answer queries in constant time by returning the distance estimate $ \delta' (x, y) $ and has the same total update time as the $ (1+\epsilon, 2) $-approximate algorithm, namely $ O ( n^{5/2} \log^2{n} / \epsilon^2 + n^{5/2} \log^4{n} / \epsilon ) $.
\end{proof}

